Localizing Moments in Long Video Via Multimodal Guidance

The recent introduction of the large-scale, long-form MAD and Ego4D datasets has enabled researchers to investigate the performance of current state-of-the-art methods for video grounding in the long-form setup, with interesting findings: current grounding methods alone fail at tackling this challenging task and setup due to their inability to process long video sequences. In this paper, we propose a method for improving the performance of natural language grounding in long videos by identifying and pruning out non-describable windows. We design a guided grounding framework consisting of a Guidance Model and a base grounding model. The Guidance Model emphasizes describable windows, while the base grounding model analyzes short temporal windows to determine which segments accurately match a given language query. We offer two designs for the Guidance Model: Query-Agnostic and Query-Dependent, which balance efficiency and accuracy. Experiments demonstrate that our proposed method outperforms state-of-the-art models by 4.1% in MAD and 4.52% in Ego4D (NLQ), respectively. Code, data and MAD's audio features necessary to reproduce our experiments are available at: https://github.com/waybarrios/guidance-based-video-grounding.

==> figures/04-experiments-fig2.tex <==
\begin{figure}[!t]
\centering
    \begin{subfigure}[t]{\linewidth}
\includegraphics[width=\textwidth]{images/legend2.pdf}
\end{subfigure}

\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\textwidth]{images/sample_a2.pdf}
\caption{“He peeks into the corridor, as a nurse walks by the reception desk.”}
\label{fig:positive_a}
\end{subfigure}

\begin{subfigure}[t]{\linewidth}
\includegraphics[width=\textwidth]{images/sample_b2.pdf}
\caption{"Someone averts his gaze from the screen and notices a man in the room.”}
\label{fig:positive_b}
\end{subfigure}

\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\textwidth]{images/negativa2.pdf}
\caption{“Cigarette hanging out of his mouth.”}
\label{fig:negative}

\end{subfigure}
\caption{\small\textbf{Qualitative Results.} We compare ground truth annotation (red box) and the predicted temporal endpoints (arrows) with their respective rankings. We highlight in blue the prediction from the baseline VLG-Net~\cite{soldan2021vlg} and in green the prediction of the baseline when combined with our guidance model. Notably, for both (a) and (b) the guidance model improves the ranking by more than 10 positions, whereas for (c) the guidance model worsens the ranking. } 
\label{fig:visualization}
\vspace{-0.5cm}
\end{figure}

==> figures/04-experiments-fig3.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\textwidth]{images/legend2.pdf}
\end{subfigure}
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\textwidth]{images/sample_non_describe2.pdf}
\end{subfigure}
\caption{\small\textbf{Filtering out non-describable moments.} We showcase how re-ranking predicted moments via our guidance model can help in ``removing'' non-describable moments from the model predictions. 
The blue and green arrows represent a VLG-Net~\cite{soldan2021vlg} moment predictions before and after the score conditioning.
This process successfully penalized the wrong prediction and improved the ranking of the baseline predictions.
} 
\label{fig:visualization2}
\vspace{-0.4cm}
\end{figure}




==> sections/01-introduction.tex <==
\section{Introduction}
\label{sec:intro}
\input{ICCV2023/figures/01-introduction-fig1}

% \noindent Audio descriptions serve not only to describe the visual content of a movie but also to capture the most critical aspects of the story being told. 
%\noindent Movie audio descriptions illustrate the most relevant visual content to the story being told. As a result, scenes and events narration are prioritized to ensure that the audience does not miss out on important details. 


%\noindent Movie audio descriptions illustrate the most relevant visual content to the story being told. As a result, scenes and events narration are prioritized to ensure that the audience does not miss out on important details. However, there may be portions of the video that are not included in the narration.  This is where a concept of a \textit{describable window} is born. 
The task of grounding natural language in long-form videos can be particularly challenging due to the possibility of encountering many video segments that do not contain any interesting or relevant moments to search for. Given the large search space, it is critical to develop approaches that can quickly scan the video and identify query-able moments via natural language. For instance, Figure~\ref{fig:teaser} shows that little activity happens in a dialogue scene that might not be related to the video's main events. At the same time, the other moments are packed with either action or descriptions that follow the context of the video's storyline. The dialogue moment, which spans more than three minutes, may be simply described as~\textit{``two people sitting on a table"}, whereas the other portion of the video contains many moments, such as \textit{``a girl falling into a pool"} and \textit{``a dog opening a fence"}, that follow the storyline of the movie. This is a clear example of why it is necessary to detect these video slices. We also argue that this observation translates to visual search scenarios, \textit{e.g.}, remarkable events such as \textit{``a dog jumps to rescue a little girl,"} are interesting moments that users would like to search for.

Datasets such as MAD~\cite{Soldan_2022_CVPR} and Ego4D~\cite{ego4d} introduce additional complexity to the task of retrieving relevant moments as multiple events may occur simultaneously. Proposal-based approaches like SSN~\cite{SSN2017ICCV} or SST~\cite{SST} would require generating several video proposals for each event class, thus not significantly reducing the computational complexity of the task. %Conversely, if a temporal window does not contain any noteworthy moment, it is referred to as a \textit{non-describable window}

Other temporal proposal techniques~\cite{AAAIYangWW0XYH22,HAN2022217,qing2021temporal} rely on simple visual cues and do not consider cues from other modalities such as audio or language (text). In addition, video-language grounding models tend to have low performance when analyzing long-form videos~\cite{Soldan_2022_CVPR}.  The above statements highlight the need to detect video slices corresponding to the ``important" parts of a long-form video, \textit{i.e.}, those that contain as many moments as possible. Our intuition is that when analyzing the entire long-form video,  grounding models might overlook the most critical segments of the video, which represents a gap in the current research and motivates us to develop  more sophisticated techniques that can capture certain intricacies using language cues or audio cues on top of the visual information.
% A \textit{describable window} refers to a video segment, a temporal window, that may contain one or more moments with a relevant storyline for the audience.
%A \textit{describable window} refers to a video segment that may contain one or more moments with a relevant storyline for the audience.

We introduce the concept of \textit{Describable windows} (Figure \ref{fig:teaser}), which are video slices shorter than the original long-form video that have a high probability of containing remarkable and relevant visual moments that can be queried through natural language. Conversely, any video slices that do not contain such visually-rich moments are considered to be \textit{non-describable windows}.

%TODO: improve this paragraph
%\noindent A significant number of non-describable windows in a movie cannot be detected solely through visual information. This poses a challenge when analyzing long-form videos; techniques such as temporal proposals~\cite{SSN2017ICCV,AAAIYangWW0XYH22,HAN2022217,qing2021temporal} fall short in addressing the problem comprehensively as they primarily rely on simple visual cues and do not consider the local narrative of the video (language modality), or even the cues from other modalities, such as audio.

%fall short in addressing the problem comprehensively. This is because these methods primarily rely on simple visual cues and do not consider the narrative of the video, or even the cues from other modalities, such as audio.
%\noindent This problem is not unfamiliar to video-language grounding models, as they tend to have low performance when analyzing long-form videos~\cite{Soldan_2022_CVPR}. Because of the non-describable windows, a large number of false positives are introduced into long-form video predictions. 
%This produces a gap in the current research and incentivizes the development of more sophisticated techniques that can capture certain intricacies, either local context of the story being told (languages cues) in a video or audio clues, particularly when considering non-describable windows. 
%\noindent Situations like conversations or static scenes may contain little visual activity, but they could be exhaustively narrated based on the video's storyline. 

Our work builds on the hypothesis that certain video segments (\textit{non-describable windows}) are difficult to narrate effectively by natural language, which can lead to noisy predictions when retrieving moments via natural language queries, particularly for long videos. In fact, state-of-the-art grounding models achieve remarkable performance when analyzing short videos~\cite{TACoS_ACL_2013, Krishna_2017_ICCV, Mun_2020_CVPR}; however, their capabilities seem to saturate when tested on longer videos~\cite{Soldan_2022_CVPR}. For example, VLG-Net~\cite{soldan2021vlg} achieves only marginal gains compared to a simple yet effective zero-shot approach~\cite{radford2021learning}, and some models even fail to achieve reasonable performance\footnote{We trained Moment-DETR~\cite{moment-detr} from scratch on the MAD~\cite{Soldan_2022_CVPR} dataset and found that, even though it achieves good grounding performance in short videos, it utterly fails in long videos. More details can be found in the supplementary material.}.

To address this issue, we propose a guided grounding framework~\cite{Hendricks_2017_ICCV, escorcia2019temporal} comprised of two core components: a \textit{Guidance Model} that specializes in filtering out non-describable windows and a base grounding model that analyzes short temporal windows to determine which temporal segments match a given query accurately. 

Observing multimodal cues is key for detecting describable windows. For instance, let us suppose we want to find the moment when~\textit{``the dog jumps to rescue the little girl''} (Figure~\ref{fig:teaser}). Here, the water splash (sound) and dog jumping (visual) are hints suggesting that lots of visual activities are happening in the scene. This intuition motivates the multimodal design of our Guidance Model. In practice, our model jointly encodes video and audio over an extended temporal window using a transformer encoder~\cite{NIPS2017_attent}.

The proposed component design balances efficiency and accuracy through our Guidance Model, which can be used in two setups: \textit{Query Agnostic} and \textit{Query Dependent}. The former pre-computes which parts of a video have a low-probability of containing describable windows, making it suitable for real-time applications or limited computational resources. In contrast, the latter provides more precise results by identifying irrelevant parts of a video based on a given text query, at the cost of being more computationally expensive as the number of queries grows. We also highlight the fact that the two-stage approach can be adapted to any grounding method, making it a flexible and versatile option for a wide range of applications.


%\noindent We design our novel component considering both efficiency and accuracy. To achieve this, our Guidance Model offers two approaches: \textit{Query Agnostic} and \textit{Query Dependent}. The \textit{Query Agnostic} approach entails pre-computing the parts of any given video that have a low probability of containing a describable moment. By pre-computing the component once, this approach is highly efficient and is useful when we need applications to run in real-time, or when we are limited by computational resources. Conversely, the \textit{Query Dependent} approach offers more precise results by enabling the identification of parts of a video that are irrelevant to a given query. When it comes to achieving high accuracy in component design, the \textit{Query Dependent} approach can be a powerful tool. This approach involves analyzing each query or input separately, allowing for a more precise result. While this method can be computationally expensive, it can lead to more accurate outcomes, making it well-suited for applications where precision is essential. Our model is also agnostic to the grounding method used in the second stage, allowing seamless integration with any method regardless of differences in modalities or training details. Our flexible and versatile model can be tailored to fit a wide range of applications and use cases, making it an ideal choice for grounding applications.

Our \textbf{contributions} are three-fold: 
\begin{enumerate}
    \item We propose a two-stage guided grounding framework: a general approach for boosting the performance of current state-of-the-art grounding models in the long-form video setting.
    \item We introduce a Guidance Model that is capable of detecting describable windows: a temporal window that contains one or more noteworthy moments.
    \item Through extensive experiments, we empirically show the effectiveness of our two-stage approach. In particular, we validate the benefits of leveraging a Guidance Model that specializes in finding describable windows. We improve state-of-the-art performance on the MAD dataset~\cite{Soldan_2022_CVPR} by $4.1\%$ and improve the performance of an Ego4D baseline model~\cite{ego4d,vslnet} in the NLQ task by $4.52\%$.
\end{enumerate}
% \textbf{(1)} we propose a two-stage guided grounding framework, a general approach for boosting the performance of current state-of-the-art video grounding models in the long-form video grounding setting; \textbf{(2)} we introduce a Guidance Model that is capable of detecting describable moments: a moment that contains anything worth describing; and \textbf{(3)} through extensive experiments, we empirically show the effectiveness of our two-stage approach. In particular, we validate the benefits of leveraging a Guidance Model that specializes in finding describable moments. We improve the state-of-the-art performance on the MAD dataset~\cite{Soldan_2022_CVPR} by $4.1\%$ and an increment of $4.52\%$ in performance using one of the Ego4D baseline models~\cite{ego4d,vslnet} in the NLQ task.


==> sections/03-method.tex <==
%------------------------------------------------------------------------
\section{Method}
\label{sec:method}
\input{figures/03-method-fig1}

\noindent\textbf{Problem Formulation.}
Given an untrimmed video $V$ and a natural language query $Q$, the video language grounding task aims to localize the temporal moment $(\tau_{s},\tau_{e})$ in the video that best aligns with the semantic content of the query. When the untrimmed video is too long and cannot be observed entirely, uniform sequential sampling is carried out using a constant window size denoted as $L_v$.
The output of grounding models, therefore, is a ranked list of $M$ moments with associated confidence scores $\{(\tau_{s},\tau_{e}, s)\}^M_1$.

% \noindent\textbf{Motivation.}
% Our main goal is to boost the performance of grounding methods in long-form settings~\cite{Soldan_2022_CVPR} by improving the ranked list of predictions.
% Current state-of-the-art methods show remarkable performance when grounding moments on short videos. However, their performance degrades when the target videos are long. The main limitations stem from the inability of existing methods to entirely process long videos due to the large computational budget requirements. Therefore, they are forced to be applied in a sliding-window fashion, leading to sub-optimal performance (i.e., prediction of many false positives). 

% \noindent To tackle this issue and bridge the performance of current methods to the long-form setup, we draw inspiration from two-step pipelines~\cite{Gao_2017_ICCV,Hendricks_2017_ICCV,MAC_WACV_2019,Liu2018AttentiveMR,WuMultimodalfusion,Song2015TVSumSW,escorcia2019temporal} and recent progress in using transformer-based architectures for multimodal understanding in images~\cite{Yao2021EfficientDI,Kamath2021MDETRM,radford2021learning} and videos~\cite{moment-detr,Akbari2021VATTTF,Li2020HeroHE,Lei2021LessIM}. 
% We propose a general two-stage guided grounding framework to boost the performance of current state-of-the-art grounding models in the long-form video grounding setup.  Our approach involves two major components: a~\textit{Guidance Model} that penalizes windows containing non-describable moments, which can lead to false positives, and a grounding model that localizes a temporal moment in a video that aligns with a given natural language query. The two models perform late fusion scoring, where new predictions are generated based on both the guidance and grounding model scores.
%It comprises two major components: a \textit{Guidance Model} that penalizes non-describable moments and a base grounding model that focuses on localizing a temporal moment in a video that aligns given a natural language query.

%------------------------------------------------------------------------
\noindent\textbf{Describable Window.} A describable window is a temporal window of length $L_{vg}$ that can contain either a single moment ($m_i$) or a set of moments $\{m\}^K_1$. Otherwise, the temporal window is considered to be a non-describable window. For an untrimmed video $V$, we can obtain a set of windows $\{W\}^N_1$. The temporal window generation is carried out through a sliding window with a stride size of $L_{vg}/2$ . \\

%-------------------------------------------------
\subsection{Pipeline Overview}
\noindent Our pipeline, outlined in Figure~\ref{fig:arch}, consists of a two-stage approach: \textbf{(i)} our Guidance Model $G$ and \textbf{(ii)} a video grounding method $V_g$. Our design is flexible and general, such that $V_g$ can be any state-of-the-art grounding model~\cite{moment-detr,Soldan_2022_CVPR,soldan2021vlg,vslnet}. The only requirement is that predictions from $V_g$ follow this structure: $\{(\tau_{s},\tau_{e}, s)\}^M_1$, where  $(\tau_{s},\tau_{e})$ corresponds to start/end time and $s$ the confidence score of the prediction. Long videos are processed in windows of length $L_v$ frames with a constant frame rate. In the following sections, we refer to \textit{moment} as any valid $(\tau_{s},\tau_{e})$ interval.  

\begin{equation}
    G(V_{g}(V,Q), V, Q^\ddagger,A^\ddagger) =  \{(\tau_{s},\tau_{e}, s^*)\}^M_1
 \label{eqn:guidance}
\end{equation}

\noindent We aim to devise an effective strategy that leverages a Guidance Model to penalize non-describable windows to rank predictions from $V_g$ more effectively. Equation~\ref{eqn:guidance} shows that the Guidance model receives as input the grounding model's output $V_{g}$, a video $V$, and setup-dependent modalities($\ddagger$): language queries ($Q$) and audio stream ($A$). The Guidance Model is tasked with computing a window-level confidence score or guidance score that measures how likely it is that a given window is \textit{describable}. The guidance scores are then combined with the grounding method's scores, producing scores $s^*$ that are used to re-rank the grounding model's predictions. The guidance method, therefore, acts as a filter, removing irrelevant chunks of videos from the search space of the grounding methods.
Finally, we adopt non-maximum suppression (NMS) to remove redundant predictions following~\cite{Soldan_2022_CVPR}. 

%------------------------------------------------------------------------
\subsection{Guidance Model}\label{sec:guidance}
\noindent The Guidance Model is depicted in Figure \ref{fig:filter}. We will review its details in the following sections. Please refer to Section \ref{sub:imple} for the implementation details. \\

\noindent\textbf{Input Representation.} 
The architecture is designed to accept diverse inputs (\textit{i.e.}, video, audio, and text). The audio and text modalities are optional and will be thoroughly ablated in Section~\ref{ablation:describabe}.  Formally, we denote video embeddings, audio embeddings, and textual embeddings as 
$E_v \in \mathbb{R}^{L_{vg} \times D_{v}}$, 
$E_a \in \mathbb{R}^{L_{ag} \times D_{a}}$, and 
$E_t \in \mathbb{R}^{L_{tg} \times D_{t}}$, respectively, where $D_{v}$, $D_{a}$, and $D_{t}$ represent the dimensionality of the features.
Input features are projected to a shared embedding space of size $d_g$ using an MLP projection followed by a layer normalization module~\cite{layernor}. Dropout is used for regularization. 

\noindent Our design allows us to configure the Guidance Model as \textit{query-dependent} or \textit{query-agnostic}. The big difference in these two setups lies in the transformer's inputs and the supervision. For \textit{query-dependent}, the transformer's inputs is $E_{in}{=}|E_{cls}, E_v, E_a, E_t| \in \mathbb{R}^{(L+1) \times d_{g}}$, where $L{=}L_{vg} + L_{ag} + L_{tg}$. Conversely, for \textit{query-agnostic} is $E_{in}{=}|E_{cls}, E_v, E_a| \in \mathbb{R}^{(L+1) \times d_{g}}$, where $L{=}L_{vg} + L_{ag} $. In both setups, a learnable CLS token is concatenated with the inputs.

%Notice that the query-agnostic approach aims at identifying all possible describable windows regardless of the input query and, therefore, can be computed only once per video, making it highly efficient. Conversely, when the textual query is part of the input, the Guidance Model has to be evaluated a new for each query, leading to more expensive yet more precise filtering results. 
\input{figures/03-method-fig2}
%\noindent The input to the Guidance Model is therefore constructed by concatenating all available modalities with a learnable CLS token. So, $E_{in}{=}|E_{cls}, E_v, E_a, E_t| \in \mathbb{R}^{(L+1) \times d_{g}}$, where $L{=}L_{vg} + L_{ag} + L_{tg}$. 

A modality-specific positional embedding is also added to each input tensor; specifically, we adopt a sinusoidal positional embedding~\cite{NIPS2017_attent} for the video modality, while we find that learnable positional embeddings~\cite{li2021learnable} work best for the audio and text modalities.\\

\noindent\textbf{Architecture.}
For the architecture design, we adopt a transformer encoder~\cite{moment-detr,Kamath2021MDETRM} which offers a powerful yet flexible architecture for processing sequential data. The input $E_{in}$ is fed to a stack of $L_{t}$ transformer encoder layers. Each transformer encoder layer is identical in design to~\cite{NIPS2017_attent,Yao2021EfficientDI,moment-detr,Kamath2021MDETRM}, using a multi-head self-attention layer and a feed-forward network (FFN). 
Finally, the first element of the encoder output $(E_{out})$, corresponding to the CLS token position, is fed to an MLP for predicting the guidance score for the given window.\\  

\noindent\textbf{Loss function and supervision definition.}
The loss function for the training process is the binary cross entropy (BCE) loss.
For supervision, describable windows are regarded as positive and non-describable windows as negative. For the query-agnostic setup, we consider a positive label if a window contains (or overlaps with) any moment of the untrimmed video, otherwise is negative. \noindent Conversely,  for the query-dependent setup only the windows that contain (or overlap) a ground truth moment associated with a given query are regarded as positive. In details, given a window $W_j{=}\left ( \tau_{w_{s}}, \tau_{w_{e}}\right )$ and ground truth $g_i{=}\left ( {\tau_{s}}', {\tau_{e}}'\right )$, we consider $W_j$ as a positive, if $tIoU(W_j, g_i)>0$, otherwise, we consider it as a negative. 

%------------------------------------------------------------------------
\subsection{Overall Score and Ranking}
\noindent Given a single moment $m_i{=}(\tau_{s},\tau_{e})$ from an untrimmed video $V$ with score $s_i$ predicted by any grounding method and a set of windows$\{W\}^N_1$ with their computed scores from the Guidance Model. We choose the most optimal score $s_j$ for the moment $m_i$ based on the window ($W_j$) of the set of windows $\{W\}^N_1$ that contains the maximum IoU with the moment $m_i$. The overall score $s^*_i$ can be described in 
equation \ref{eqn:score}.
\begin{equation}
    s^*_i = s_i * s_j \,\, \text{where} \,\,\,  j = \argmax(tIoU(m_i,\{W\}^N_1))
\label{eqn:score}
\end{equation}
Lastly, temporal moments are re-ranked according to the new score, and non-maximum suppression (NMS) is applied to remove redundant predictions.


==> sections/07-rebuttal.tex <==
%\noindent We thank the reviewers for their valuable comments and constructive feedback. We are encouraged they found our motivation and idea to be a novel and sufficient contribution to the research community (\textbf{\textcolor{red}{R1}}, \textbf{\textcolor{green}{R3}}). We are glad they found our approach is supported by extensive ablation studies~(\textbf{\textcolor{blue}{R2}}, \textbf{\textcolor{green}{R3}}). Furthermore, we are glad that \textbf{\textcolor{red}{R1}} acknowledges the model-agnostic nature of our approach, and \textbf{\textcolor{green}{R3}} recognizes its superior performance in long-form video benchmarks. We address reviewers comments below and we will incorporate all the feedback.
\noindent We thank the reviewers for acknowledging the relevance of our motivation and approach (\textbf{\textcolor{red}{R1}}, \textbf{\textcolor{green}{R3}}), and the extensive ablation studies supporting our design (\textbf{\textcolor{blue}{R2}}, \textbf{\textcolor{green}{R3}}). 
% The discussion unfolds as follows:

% We appreciate the reviewers' valuable comments and feedback. They found our motivation and idea to be novel and significant (\textbf{\textcolor{red}{R1}}, \textbf{\textcolor{green}{R3}}). The reviewers also acknowledged the extensive ablation studies supporting our approach (\textbf{\textcolor{blue}{R2}}, \textbf{\textcolor{green}{R3}}). The discussion unfolds as follows:

\noindent \textbf{\textcolor{red}{(R1-Q4,Q5)} Multimodal Models.} We considered several multimodal architectures to validate the model-agnostic nature of our approach: CLIP (multi-modal vision and language model) in a zero-shot setup, VLG-Net (video-language graph network), Moment-DETR (\textbf{multimodal transformer} encoder/decoder), and VSL-Net (span-based QA framework). This flexibility allows for future improvements by incorporating new SOTA into our method. Yet, our focus lies on the two-stage approach concept validation.


\noindent \textbf{\textcolor{red}{(R1-Q3)} Audio grounding.}  By incorporating audio features in Moment-DETR, we observed a significant performance boost. In Tab.~\ref{tab:ground_audio}, mR$_{all}$ improves from $5.08\%$ to $7.70\%$. When combined with the guidance model,  mR$_{all}$ grows from $24.19\%$ to $28.30\%$, showing a consistent boost. We will include this ablation in our main paper, showcasing the first audio-visual grounding model for the task.
% the performance improved from $5.08\%$ to $7.70\%$ in mR$_{all}$, and with Guidance, it increased from $24.19\%$ to $28.30\%$ in mR$_{all}$. The performance boost in video grounding inspires our future work on novel grounding architectures combining audiovisual and text data.

\noindent \textbf{\textcolor{red}{(R1-Q2)} Guidance Ablation.} We use the guidance model for both first stage and second stage. We observe that this model provides good performance for low IoUs while fails at higher ones (R@1-IoU=0.1: $7.24\%$, R@1-IoU=0.5: $0.08\%$). This aligns with our design, where the guidance can only provide a coarse alignment, while the grounding model is used to predict fine-grained alignment. 

\noindent \textbf{\textcolor{blue}{(R2-Q2)} Unfair comparison with SOTA.}  Our evaluation in Tab.1 (main paper) is fair as all grounding methods have access to visual and textual features only. In the main paper, only the guidance model has access (optionally) to audio features, which prove to be beneficial. The same guidance model is paired with each grounding method, ensuring fairness. We will review our manuscript to improve clarity. 

% , we present the performance of grounding baselines without audio features. However, when combined with our Guidance Model in the most effective setting (query-dependent with video, audio, and text modalities), all baselines benefit from this technical modification. Thorough ablation studies on the guidance model are provided in Tab. 3 and 4. Importantly, incorporating audio features in the guidance model does not impact the fairness of our comparisons with any grounding model. 
% \textcolor{red}{Reference that table 2 is for guidance + grounding and we are missing the T. }
% We suspect that the reviewer may have misunderstood our evaluation protocol. In Tab. 1 (main paper), we present the performance of grounding baselines, where none of the methods utilize audio features. However, when these baselines are combined with our Guidance Model in its most effective setting (query-dependent with video, audio, and text modalities), we observe that this technical modification proves beneficial for all baselines. We further provide thorough ablation studies on the guidance model in Tab. 3 to 4. It's important to note that the inclusion of audio features in the guidance model does not impact the fairness of our comparisons when combined with any grounding model.

\noindent \textbf{\textcolor{blue}{(R2-Q3)} Common baseline between benchmarks.} Following the suggestion, we use Moment-DETR as a common baseline and report results in Tab.~\ref{tab:egod4reb}.
The combination of our guidance model with the baseline grounding model leads to performance improvements in both datasets. Notably, we observed that the guidance model has a larger impact on longer videos, resulting in greater improvements in MAD (${\sim}110$ minutes per video) compared to Ego4D (${\sim}8$ minutes per video). These findings further validate the effectiveness of our framework, as emphasized by \textbf{\textcolor{red}{R1}} and \textbf{\textcolor{green}{R3}}.
% As acknowledged by \textbf{\textcolor{red}{R1}} and \textbf{\textcolor{green}{R3}}, our approach is effective. 
% improved Moment-DETR by $1.32\%$ and boosted VSL-Net by $4.52\%$ in Table~\ref{tab:egod4reb}. These results reinforce the effectiveness of our framework, as highlighted by \textbf{\textcolor{red}{R1}} and \textbf{\textcolor{green}{R3}}.


%Our pipeline is flexible with any grounding model, as recognized by \textbf{\textcolor{red}{R1}}. In our experiments on the MAD dataset, we showcased the advantages of our guidance model with three different grounding models: zero-shot, proposal-based, and proposal-free. The VSL-Net further supports the applicability of our approach to long-form videos overall. This strengthens the framework's effectiveness, as highlighted by \textbf{\textcolor{green}{R3}}. Grounding methods are dataset-specific and may not translate equally well to different video domains, which is an open research question. However, this does not undermine our results and contributions.


\noindent \textbf{\textcolor{blue}{(R2-Q1)} Inference Time.} Tab.~\ref{tab:reb1} shows the inference time for each baseline and guidance model. The agnostic setup is tailored for low computational budgets, as it performs a single sliding-window forward pass per movie ($112$ movies). Conversely, the query dependent setup requires a number of forward passes that is directly proportional to the number of queries ($72k$) and temporal windows. Note that we can further reduce inference time by using the guidance model to filter out windows prior to grounding, depending on which of recall or precision is more important.%we found that using all predictions from both models allowed us to consider 

\noindent \textbf{\textcolor{blue}{(R2-Q4)} Visualizations and additional analysis.} The improvement in the R@1 metric when combining our guidance model with the baseline grounding methods is directly related to boosting low-scoring predictions to the top of the ranking list; \textit{e.g.}, on MAD with VLG-Net the R@1-IoU=0.1 grows from $3.5$ to $5.6$. %(around $2,500$ windows for which the GT query is pushed to the top). 
Additional breakdown of these metrics will be included in the appendix along with additional visualizations for the Ego4D dataset. 

%We thank the reviewer for his/her acknowledgment of our multiple relevant contributions to the community. We will reflect his/her feedback in our introduction.

\noindent\textbf{\textcolor{green}{(R3-Q1)} Training datasets for Query Agnostic vs Dependent.} Positive and negative windows are defined differently in each setup. In the query-agnostic setup, a window is positive if it contains any annotation, and negative otherwise. At training time, a window is sampled randomly and the model is tasked with predicting if such window is positive or negative.  In the query-dependent setup, a window is positive only if it contains the ground truth moment for the given sentence, while all others are negatives. During training, a random window is sampled and the model predicts if it is relevant for the query or not. We will review our manuscript to improve clarity.
%\input{ICCV2023/tables/07-rebutal-audio} 
\input{ICCV2023/tables/07-rebuttal-tab1} 
\input{ICCV2023/tables/06-appendix-tab5} 
\input{ICCV2023/tables/06-appendix-audio}

\noindent \textbf{\textcolor{green}{(R3-Q2)} Describable Windows.} 
In lines 117-123 (main paper), we introduce the concept of ``describable windows''. 
% which refers to short video segments extracted from long-form videos that are likely to contain significant and relevant moments that can be queried using natural language. 
This concept is general and applicable to any long-form video dataset. We specifically use two long-form datasets from different domains (movies and egocentric videos) to demonstrate the versatility of our method. However, we do not address cross-dataset generalization on them as it poses unique challenges due to contrasting camera perspectives (i.e., 1st person in Ego4D, and 3rd person in MAD). 


\noindent\textbf{(\textcolor{red}{R1},\textcolor{blue}{R2},\textcolor{green}{R3}) Editorial.} We will incorporate the reviewers' feedback in the camera-ready version: social impact and beyond two-stage contribution.


==> tables/07-rebuttal-tab1.tex <==
\begin{table}[t]
\vspace{.1cm}
\centering
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1} 
\resizebox{1\columnwidth}{!}{%
\footnotesize
\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
& \multicolumn{4}{c}{\textbf{Ego4D Dataset}} & \multicolumn{4}{|c}{\textbf{MAD Dataset}} \\
\textbf{Method} & 
\textbf{mR@1} & \textbf{mR@5} & \textbf{mR@10} & \textbf{mR@50} &
\textbf{mR@1} & \textbf{mR@5} & \textbf{mR@10} & \textbf{mR@50} 
\\ \midrule

Moment-DETR
& $6.72$ 
& $19.68$ 
& $23.85$ 
& $24.67$ 
& $0.24$
& $1.11$
& $2.02$
& $7.92$
% & $14.13$
\\

\midrule

$\dagger$Moment-DETR
& $\mathbf{7.28}$ 
& $\mathbf{22.14}$ 
& $\mathbf{24.75}$ 
& $\mathbf{26.05}$ 
& $\mathbf{3.76}$
& $\mathbf{12.27}$
& $\mathbf{18.76}$
& $\mathbf{38.48}$
% & $\mathbf{47.65}$
\\
				

\bottomrule
\end{tabular}
}
\vspace{.001cm}
\caption{\footnotesize{\label{tab:egod4reb}{\bf Common baseline across datasets.}  We highlight the methods employing the guidance model with $\dagger$.}}
\vspace{-.3cm}
\end{table}


% \begin{table}[t]
% \vspace{.1cm}
% \centering
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{1} 
% \resizebox{\columnwidth}{!}{%
% \footnotesize
% \begin{tabular}{@{}lllllllll@{}}
% \toprule
% \multicolumn{3}{l}{\textbf{Method}} & \textbf{mR@1} & \textbf{mR@5} & \textbf{mR@10} & \textbf{mR@50} & \textbf{mR@100} & \textbf{mR$_{all}$} \\ \midrule
% \multicolumn{3}{l}{VSL-Net} & $11.38$ & $19.64$ & $24.27$ & $36.09$ & $42.12$ & $26.70$\\
% \multicolumn{3}{l}{Moment-DETR} & $6.72$ & $19.68$ & $23.85$ & $24.67$ & $-$ & $18.73$\\\midrule
% \multicolumn{3}{l}{$\dagger$VSL-Net} & $\mathbf{11.90}$ & $\mathbf{24.06}$ & $\mathbf{33.31}$ & $\mathbf{54.59}$ & $\mathbf{54.90}$ & $\mathbf{31.22}$ \\
% \multicolumn{3}{l}{$\dagger$Moment-DETR} & $7.28$ & $22.14$ & $24.75$ & $26.05$ & $-$ & $20.05$\\

% \bottomrule
% \end{tabular}
% }
% \vspace{-.1cm}
% \caption{\small\label{tab:egod4reb}{\bf Benchmarking on Ego4D.} Refactored Table. We highlight the methods employing the guidance model with $\dagger$.}
% \end{table}


